ChartGalaxy++: A Richly Annotated Dataset for Chart Understanding and Generation

Infographic charts communicate data through cohesive compositions of visual elements such as charts, text, and images. Existing infographic chart datasets primarily annotate individual elements with bounding boxes and category labels. Such element-level annotations do not capture hierarchical and spatial relationships, limiting their use for understanding how elements are organized and related within an infographic and for generating well-organized designs. To address this limitation, we introduce ChartGalaxy++, a richly annotated dataset of 217,195 infographic charts. At the core of this dataset is a scene graph representation, in which nodes represent visual elements and semantic groups, and edges encode their hierarchical and spatial relationships. For real infographics, we construct scene graphs by detecting and progressively grouping visual elements; for synthetic ones, we derive them directly from the generation process. We demonstrate the utility of ChartGalaxy++ through three applications: 1) image-to-scene-graph prediction, 2) scene-graph-augmented infographic question answering, and 3) evaluation of scene graph preservation in image generation. Together, these applications highlight the value of ChartGalaxy++ for advancing chart understanding and generation.

==> 1-introduction-old.tex <==
\section{Introduction}
\label{sec:introduction}

% 第一段：background and problem
% infographic chart定义以及优点
Infographic charts combine charts with text and images to create cohesive visual designs.
By presenting complex data in an accessible and compelling manner, they have become pervasive in real-world applications, such as news reporting, business communication, and public education~\citep{cui2022mixed,elaldi2021effectiveness}.
% 研究问题：信息图表的复杂性给模型的理解和生成带来的困难。
Despite these benefits, the visual and structural richness of infographic charts makes them challenging for foundation models to understand and generate.
% 具体解释：理解中的问题
For example, even frontier LVLMs such as GPT-5.6~\citep{openai2026gpt56} still struggle to locate relevant evidence in complex charts, integrate information across visual elements, and perform reliable multi-step reasoning over the underlying data~\citep{masry2025chartqapro,bansal2025chartab,efat2026polychartqa,xiao2026longchart}.
% 具体解释：生成中的问题
Moreover, Nano Banana Pro~\citep{google2025nanobananapro} can produce visually appealing outputs but still struggles to faithfully encode the underlying data, render textual and visual content accurately and completely, and organize these elements into coherent designs~\citep{tang2026igenbench}.


Recent work has shown that fine-grained annotations that go beyond chart-level descriptions to encode element-level descriptions, bounding boxes, and relationships can improve visually grounded reasoning and enable more precise control over layout and style during generation~\citep{zhu2026infodet,gutflaish2025structuredcaptions,reve2026layoutbet,ideogram2026ideogram4}.
% 引出研究挑战和数据需求
These findings motivate the need for large-scale, high-quality infographic-chart data with such fine-grained annotations.
% 转到对现有工作的讨论。
However, existing datasets only partially meet these requirements.
% 收集+标注数据集的局限性
Existing infographic datasets collected from real-world sources remain limited in scale, and even producing reliable annotations of element boxes requires substantial manual effort~\citep{zhu2026infodet}.
% 目前生成数据集的局限性
Synthetic datasets such as \chartgalaxy{} achieve substantially greater scale and exact data grounding, but their design space remains constrained by a fixed set of layout templates and manually implemented chart variations~\citep{li2026chartgalaxy}.
% 总结
Consequently, existing datasets do not yet combine scale, broad design coverage, reliable data grounding, and fine-grained annotations.

To address this gap, we introduce \dataset{}, a large-scale infographic-chart dataset that extends \chartgalaxy{} in both design coverage and annotation granularity.
We construct \dataset{} using a pipeline with two components: 1) expert-guided expansion of chart variation and 2) scene-graph-guided layout construction.
First, expert-guided agents automate chart variation coding, reducing the manual implementation effort required in ChartGalaxy and enabling a larger and more diverse library of chart variations while preserving valid visual encodings.
Second, \dataset{} extends beyond the layout templates in \chartgalaxy{} by using scene graphs to represent layouts with more elements and richer structural relationships and to provide fine-grained annotations for the resulting infographic charts.
The resulting dataset contains \totalnum{} infographic charts paired with fine-grained scene-graph annotations.

We demonstrate the utility of \dataset{} through three representative applications, each highlighting a distinct aspect of its value.
First, to evaluate fine-grained infographic-chart understanding, we introduce an image-to-scene-graph reconstruction task that requires models to recover individual elements and their structural relationships from raster images.
Second, we construct a benchmark for fine-grained infographic-chart editing that evaluates whether models can modify the content, appearance, or position of selected elements while preserving the rest of the design.



